AnoRand: A Semi Supervised Deep Learning Anomaly Detection Method by Random Labeling

Anomaly detection or more generally outliers detection is one of the most popular and challenging subject in theoretical and applied machine learning. The main challenge is that in general we have access to very few labeled data or no labels at all. In this paper, we present a new semi-supervised anomaly detection method called \textbf{AnoRand} by combining a deep learning architecture with random synthetic label generation. The proposed architecture has two building blocks: (1) a noise detection (ND) block composed of feed forward ferceptron and (2) an autoencoder (AE) block. The main idea of this new architecture is to learn one class (e.g. the majority class in case of anomaly detection) as well as possible by taking advantage of the ability of auto encoders to represent data in a latent space and the ability of Feed Forward Perceptron (FFP) to learn one class when the data is highly imbalanced. First, we create synthetic anomalies by randomly disturbing (add noise) few samples (e.g. 2\%) from the training set. Second, we use the normal and the synthetic samples as input to our model. We compared the performance of the proposed method to 17 state-of-the-art unsupervised anomaly detection method on synthetic datasets and 57 real-world datasets. Our results show that this new method generally outperforms most of the state-of-the-art methods and has the best performance (AUC ROC and AUC PR) on the vast majority of reference datasets. We also tested our method in a supervised way by using the actual labels to train the model. The results show that it has very good performance compared to most of state-of-the-art supervised algorithms.

==> supervised.tex <==


\subsection{Supervised case architecture}
In the supervised framework, we have access to to training features and the corresponding labels so we don't need to generate synthetic labels. Unlick the unsupervised architecture, in the supervised case, the MLP part plays a central place in the final prediction. Recall that in the unsupervised framework, the MLP block has a simple role of informing and reinforcing the capacity of the autoencoder to embed the normal samples. In the supervised scenario, the two block are more tied and the MLP block uses the auto encoder latent block as a hidden layer. The final prediction is the output of the MLP part of the model. 
\subsubsection{Supervised Final loss function}


The loss function is defined as follows:
\begin{equation}
\label{loss_unsup}
   loss = CE\cdot (1-w)+ w\cdot MAE
\end{equation}

Unlike the unsupervised scenario, in the supervised case, the final loss is mainly impacted by the cross entropy loss of the MLP part. 

